Learning Causal Graphs with Small Interventions

We consider the problem of learning causal networks with interventions, when each intervention is limited in size under Pearl's Structural Equation Model with independent errors (SEM-IE). The objective is to minimize the number of experiments to discover the causal directions of all the edges in a causal graph. Previous work has focused on the use of separating systems for complete graphs for this task. We prove that any deterministic adaptive algorithm needs to be a separating system in order to learn complete graphs in the worst case. In addition, we present a novel separating system construction, whose size is close to optimal and is arguably simpler than previous work in combinatorics. We also develop a novel information theoretic lower bound on the number of interventions that applies in full generality, including for randomized adaptive learning algorithms. For general chordal graphs, we derive worst case lower bounds on the number of interventions. Building on observations about induced trees, we give a new deterministic adaptive algorithm to learn directions on any chordal skeleton completely. In the worst case, our achievable scheme is an $\alpha$-approximation algorithm where $\alpha$ is the independence number of the graph. We also show that there exist graph classes for which the sufficient number of experiments is close to the lower bound. In the other extreme, there are graph classes for which the required number of experiments is multiplicatively $\alpha$ away from our lower bound. In simulations, our algorithm almost always performs very close to the lower bound, while the approach based on separating systems for complete graphs is significantly worse for random chordal graphs.

==> Sepsys.tex <==
Given a set $X$ of $n$ variables $X=\{X_1,X_2,...,X_n\}$, $\mathcal{S}=\{S_1,S_2,...,S_m\},S_i\subseteq X$ is a separating system for $X$ if for every $i,j\in[n]$, there exists $k\in[m]$ such that either $X_i\in S_k$ and $X_j\notin S_k$ or $X_i \notin S_k$ and $X_j\in S_k$. In words, a set of subsets is a separating system if for every pair of elements, there is a subset that separates them. When each element of $\mathcal{S}$ has cardinality constraint of $k$, $\mathcal{S}$ is called a $k-$separating system.

In \cite{Katona1966}, Katona gave a $k-$separating system together with a lower bound on the minimum size of a $k-$separating system. In \cite{Wegener1979} Wegener tightened gave a simple information theoretic argument for the lower bound and also provided a much simpler construction as an achievable scheme, which performs better than Katona's. We give a construction which achieves the same number of sets as Wegener's, however it is a simpler construction, and it can be easily extended to generalized separating systems on graphs.



==> prevwork.tex <==
When the intervention size is unbounded, \cite{Hauser2012b} finds an efficient algorithm for any chordal graph that minimizes the number of experiments in the worst case. The algorithm is based on optimal coloring of chordal graphs, which can be done in polynomial time. This approach does not seem to generalize to size$-k$ intervention setting.

Studies on fully identifying the causal DAG using size $k$ interventions are limited. The first work we are aware of in this regime is by Eberhardt, where he provided an achievable scheme in \cite{Eberhardt2005}. %, which he also claimed to be necessary in the worst case. However, this bound is not necessary as he corrected in his thesis \cite{EberhardtThesis}.  
He proved in \cite{EberhardtThesis} that the set of interventions to fully identify the causal DAG needs to be a separating system for the set of variables, when the intervention size is not constrained or is 1. In \cite{Hyttinen2013}, with the assumption that the same holds true for any intervention size, Hyttinen draws connections between the combinatorics literature and causality via known separating system constructions. The proof of whether one still needs a separating system for interventions of size $k$ in the worst case was not known until this work although highly suspected to be true \cite{EberhardtPersonal}. 

%Following the line of work by Eberhardt, we first show that the set of size$-k$ experiments should correspond to a separating system in the worst case setting. In particular, we show that there exist DAGs over the complete graph, which can force the set of experiments to be a separating system in the constrained intervention setting. Later, we provide a simple construction for a $k-$separating system. Our construction gives the same size as the best known construction \cite{Sep2} and is much simpler. Additionally, this construction allows us to extend the $k-$separating system notion to general chordal graphs. We give the first $k-$separating system on any chordal graph. We provide a simple lower bound on the number of experiments necessary to fully identify the whole causal DAG and use this lower bound  to show that our construction in for chordal graph achieves an approximation ratio of $\alpha$, where $\alpha$ is the independence number of the chordal graph. This construction is later improved to give better bounds, which uses not only the maximum independent set, but the sizes of all the independent sets in an optimal coloring. Finally, we give a heuristic algorithm that uses Meek rules to identify additional edges, while guaranteeing the optimal discovery of large cliques. We evaluate this algorithm in simulations.

%RANDOMIZED?ARE WE ADDING OUR RANDOMIZED ALSO?
%In \cite{Hu2014}, the first randomized algorithm for causal discovery is proposed. The authors first consider a complete graph. With the help of randomization, the \emph{worst case DAG} can be avoided and it is shown that $O(\log\log n)$ experiments are sufficient to identify the causal DAG with polynomially small error probability. The result carries over to any chordal graph, since chordal graphs have at most $n$ maximal cliques. However, the algorithm uses size$-n/2$ interventions, and it is not clear if the results hold for size$-k$. We build on their ideas to provide a similar result for size$-k$ interventions on the complete graph and show that...



%Even though the Bayesian network of a probability distribution is not, a causal Bayesian network is unique. This relation is important to understand what can be learned about the causal DAG using only the observational data, i.e., the conditional independence queries between the variables.


%A DAG is a causal Bayesian network, if it encodes the post-intervention distribution. 


%Formally, a Bayesian network for a set of variables $X=\{X_1,X_2,...,X_n\}$ is a pair $(D,\mathcal{P})$, where $D=(V,E)$ is a DAG with a one-to-one labeling $\sigma:X\rightarrow V$, and $\mathcal{P}=\{p_1,p_2,...,p_n\}$ is a set of local conditional probability distributions for each vertex of $D$ \cite{Heckerman96}. Without loss of generality, assume $\sigma$ is identity. Each $p_i$ depends on $Pa(X_i)$, i.e., the variables in the parent set of $X_i$. Then the joint distribution of $X$ can be written as $p(x)=\prod\limits_{i=1}^n p_i(x_i|Pa(x_i))$, where $x_i$ is an evaluation of variable $X_i$ and $Pa(x_i)$ stand for an evaluation of the parent set of $X_i$.




%ASSUMPTIONS: In this work, we assume that a conditional independence query is available. Hence, the results are true in the large sample limit, where CI queries are reliable. We assume that the observational data is available. Hence, observational essential graph can be obtained using any existing algorithm, such as the PC algorithm \cite{Spirtes2001}. We also assume that the post-intervention distribution is similarly available. These assumptions reliefs the causal learning problem from its statistical peculiarities and reduces it to a graph learning algorithm based on intervention queries and iterative application of Meek rules.

%Essential graph learning algorithms can be used after an intervention to identify the interventional essential graph. The objective of active causal learning is to minimize the number of interventions in the worst case that lead to full idenifiabiliy of the causal DAG. Worst case refers to the fact that optimization minimizes maximum the number of interventions over all DAGs. We consider interventions of size at most $k$. Let $\ess(D_0)$ be the essential graph of the underlying DAG $D_0$, and ${V\choose k}$ stand for the subsets of $V$ of size at most $k$. Then the objective is to find   
%\begin{equation*}
%\begin{aligned}
%\mathcal{I}^*=&\argmin\limits_{\mathcal{I}\in {V \choose k}^N}\max\limits_{D \in [D_0]} & N &\\
%&\text{\hspace{.15in}subject to } &\ess_{\mathcal{I}}(D)&=D_0 
%\end{aligned}
%\end{equation*}

%In the following sections, for complete essential graphs we simplify this problem by showing that there are DAGs which require the set of interventions to fully identify the DAG to correspond to a \emph{separating system} for the set of nodes of the graph. Hence, the above problem reduces to finding separating systems with size-k sets, which has been studied in the combinatorics literature before.



